DyTox: Transformers for Continual Learning with DYnamic TOken eXpansion

Deep network architectures struggle to continually learn new tasks without forgetting the previous tasks. A recent trend indicates that dynamic architectures based on an expansion of the parameters can reduce catastrophic forgetting efficiently in continual learning. However, existing approaches often require a task identifier at test-time, need complex tuning to balance the growing number of parameters, and barely share any information across tasks. As a result, they struggle to scale to a large number of tasks without significant overhead. In this paper, we propose a transformer architecture based on a dedicated encoder/decoder framework. Critically, the encoder and decoder are shared among all tasks. Through a dynamic expansion of special tokens, we specialize each forward of our decoder network on a task distribution. Our strategy scales to a large number of tasks while having negligible memory and time overheads due to strict control of the parameters expansion. Moreover, this efficient strategy doesn't need any hyperparameter tuning to control the network's expansion. Our model reaches excellent results on CIFAR100 and state-of-the-art performances on the large-scale ImageNet100 and ImageNet1000 while having less parameters than concurrent dynamic frameworks.

==> content/exp_backup.tex <==
\section{Experiments}
\label{sec:exp}

\begin{comment}
\begin{figure}[t!]
\centering
  \includegraphics[width=1\linewidth]{images/nb_params.png} 
    \caption{Number of parameters w.r.t number of tasks for DER \cite{yan2021der}, DER without pruning \cite{yan2021der}, and ours (DyTox). Note that our ensemble method has a minimal parameters grows (+384 / per task) while also requiring no advanced hyperparameter tuning like DER does.}
\label{fig:nb_params}
\end{figure}
\end{comment}

\subsection{Benchmarks \& Implementation}

\noindent\textbf{Benchmarks \& Metrics} We evaluate our model on CIFAR100 \cite{krizhevskycifar100}, ImageNet100 and ImageNet1000 \cite{deng2009imagenet} (datasets description in the supplementary materials) under different settings, where for each the number of new classes seen per step is different. Therefore, in CIFAR100, we evaluate our model on 10 steps (10 new classes per step), 20 steps (5 new classes per step), and 50 steps (2 new classes per step). The same logic applies to ImageNet100 10 steps (10 new classes per step) and ImageNet1000 10 steps (100 new classes per step). \alex{d'abord présenter ImageNet, qui est le dataset principal, puis CIFAR}. We compare models using the top-1 accuracy \alexd{on CIFAR100 and ImageNet}{inutil, à supprimer, ça laisse entendre qu'il y a d'autres datasets}. We also use top-5 accuracy on ImageNet. \alex{In addition to the top-1 accuracy, we also use the top-5 on ImageNet}. We report the ``\textit{Avg}'' accuracy which is the average of the accuracies after each step as defined by \cite{rebuffi2017icarl}. We also \alexd{choose to}{} report the final accuracy after the last step (``\textit{Last}''). Finally ``\textit{\#P}'' denotes the parameter count in million at the final step \alexd{at test-time}{pourquoi at test ? qu'est ce qui change en train ? c'est pour le pruning ? si oui, pas besoin}.

\input{tables/transf_archi}
\input{tables/imagenet}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{images/imagenet100.png}
    \caption{\textbf{Performance evolution on ImageNet100}. The top-5 accuracy (\%) is reported after learning each task. Our model DyTox (in \textbf{\textcolor{red}{red}}) surpasses significantly most baselines, and is of equal performance as the complex DER that uses pruning with setting-specific hyperparameters. \alex{remettre les poids dans la FIgure 1, non ?}}
    \label{fig:imagenet100}
\end{figure}
\noindent\textbf{Implementation details} \alex{please des paragraphes ... trop serré} Our network architecture \alexd{is the same for all datasets and }{has similar structure hyperprameter as} defined in \autoref{tab:archi}. We use 5 Self-Attention Blocks (SABs), 1 Task-Attention Block (TAB). All 6 have an embedding dimension of 384 and 12 attention heads. We use the attention with spatial prior introduced by ConViT \cite{dascoli2021convit} for all SABs\alex{. Its prior}{which} allows training transformers on a small dataset (like CIFAR) without needing pretraining on large datasets or \alexd{using}{inutil} complex regularizations. We use for all models (baselines included) 2,000 \alex{c'est standard comme chiffre? citation} images of rehearsal memory for CIFAR100 and ImageNet100, and 20,000 images for ImageNet1000. 
%For all settings that starts with 50 initial classes, the memory is fixed per class, while for other settings the memory is fixed in total.
The implementations of the continual scenarios are provided by Continuum \cite{douillardlesort2021continuum} and our \alexd{code}{implementation, code est repeté juste apres} is based on the DeiT \cite{touvron2021deit} code base which itself uses extensively the timm library \footnote{available at \url{http://github.com/rwightman/pytorch-image-models/}}. We'll release publicly our code to facilitate the reproduction of our results \alex{important: faudrait faire un repo anonym. Même donner l'url dans l'abstract/intro. Ca changera des DER}. The full implementation details can be found in the supplementary materials.

\input{tables/cifar100_b0}

\begin{figure*}[t!]
\centering
  \includegraphics[width=0.9\linewidth]{images/cifar.png}
    \caption{Accuracy for each step on the CIFAR100 dataset. \textbf{Left} is evaluated with 10 steps, \textbf{middle} with 20 steps, and \textbf{right} 50 steps.}
\label{fig:increment_cifar}
\end{figure*}

\subsection{Quantitative results}

\alex{paragraph à restructurer. Ca part dans tous les sens}
\noindent\textbf{ImageNet}:\,We report in \autoref{tab:imagenet} performances of all models on ImageNet100 (10 steps), and ImageNet1000 (10 steps) \alex{always 10 steps, pas besoin de lre dire 2 fois}. In ImageNet100, DyTox outperforms the pruned DER$^\dagger$ by +2.5\% in ``Last'' accuracy.
%Our main concurrent, DER, has less significant gain in this 10-steps ImageNet100 compared to the 10-steps CIFAR100, and their pruning procedure is also less effective (4.96M vs 7.67M).
\alexd{DER proposed a pruning method to reduce that amount to an acceptable level; unfortunately, this pruning required a different hyperparameter tuning for each setting. We denote by a $^\dagger$ the DER with setting-specific pruning, and \textit{w/o P} for the DER without pruning. Simple-DER also uses pruning but without the need of hyperparameter tuning.}{à mettre dans implementation details}
\alexd{ImageNet data is more complex than CIFAR (image sizes are 32$\times$32 vs 224$\times$224) and the image diversity is significantly higher: as a result DER struggles to scale and its pruning is less efficient than on CIFAR (detailed later).}{à mettre dans dataset introductin} On the other hand, our model DyTox is able to scale correctly to this complex large-scale dataset, with a higher performance gain (67.76\% in ``Last'' for ImageNet100 vs DER's 66.06\%) while handling seamlessly the parameter growth. \alexd{DyTox has slightly more parameters on ImageNet than on CIFAR (11.014M vs 10.687M) for an equal amount of steps because more patch tokens exist for the former dataset resulting in bigger learned positional embeddings in the tokenizer}{à mettre dans implementation details}. This overhead is however minimal, and the parameter count between ImageNet100 and ImageNet1000 doesn't change while DER grows +89\% more (7.67M vs 14.52M). On ImageNet1000, despite learning ten times more classes, DyTox scales well to this challenging task, and outperforms all other models on all metrics: even DER without pruning (``\textit{w/o P}'') with 10 ResNet18 in parallel and 61.6m parameters has lower performance. \alexd{DyTox, by sharing early layers, has a much lower parameters count (11.014M) and is able to put in common class-agnostic features \cite{olah2017feature} for all tasks}{déjà présent après dans computation overhead}. We illustrated in \autoref{fig:imagenet1000} all models evolutions on ImageNet1000: DyTox constantly surpasses previous state-of-the-art models despite having comparable performance at the first step. The same figure for ImageNet100 is displayed in \autoref{fig:imagenet100}. \alexd{faut que ça pete ! tes résultats sont dingues, mets les en avant}

\noindent\textbf{CIFAR100}:\, We report in \autoref{tab:cifar100-b0} results \alexd{of the baselines and our model}{for all approaches} on CIFAR100. All settings have an equal amount of new classes per step (resp. 10, 5, and 2 classes per step for 10 steps, 20 steps, and 50 steps). The more steps there are, the larger is the forgetting and thus the lower is the performance. 
%RPSNet \cite{rajasegaran2019rpsnet} and DER \cite{yan2021der} have a large number of parameters because of their dynamic strategy.
% https://github.com/Rhyssiyan/DER-ClassIL.pytorch/issues/4#issuecomment-865853428
%This is unrealistic because in a true continual learning, we aren't supposed to know the number of future classes and thus the same hyperparameters should be applied to all settings of a same dataset. 
\alexd{We tuned the hyperparameters of DyTox for CIFAR100 10 steps, and then kept them fixed for all other settings, ImageNet included.}{important: mettre en gras ? en avant dans implementation details peut être} \alexd{Furthermore, our dynamic strategy doesn't require any complex pruning because the memory overhead per task (see \autoref{sec:memory_overhead}) is very small: Our base network has 10.684M parameters, 10.687M with 10 class tokens, and 10.702M with 50 class tokens}{cf autres remarques}. DyTox is in every setting close to ``DER without pruning'' (\textit{w/o P}) performance for much fewer parameters (up to 26x less) and significantly above other baselines (up to +25\% in ``Last'' accuracy in 50 steps). 

\noindent\textbf{Improved Training Procedure:} Finally, we propose an efficient training procedure for continual learning which proved to greatly reduce catastrophic forgetting. We generate continuously novel images by linear interpolation of existing images using MixUp \cite{hingyi2018mixup}. The interpolation factor is sampled $\lambda \sim \operatorname{Beta}(\alpha, \alpha)$ and then the pixels of two images are mixed ($x = \lambda x_1 + (1 - \lambda) x_2$) as their labels ($y = \lambda y_1 + (1 - \lambda) y_2$). MixUp has two main effects: (1) it diversifies the training images and thus enlarges the training distribution on the vicinity of each training sample \cite{chapelle2001vicinalrisk} and (2) it improves the network calibration \cite{guo2017miscalibration,thulasidasan2019mixupcalibration}, reducing the overconfidence in recent classes and in turn reducing the forgetting of older classes. It further emphasizes the re-calibration already induced by the sigmoid activation  \cite{belouadah2019il2m,wu2019bias_correction}, \alexd{but we highlight the seamless calibration through training via MixUp which adds no overhead contrary to previous works}{at no overhead, le reste n'apporte pas d'info }. When DyTox is combined with our novel continual training procedure, nicknamed as \textit{DyTox+} \alex{pourquoi italic}, our model improves state of the art in \textit{Avg} by a significant margin in all three settings of \autoref{tab:cifar100-b0}. Those settings are also displayed in \autoref{fig:increment_cifar} where model performances are displayed after every step. Again, the excellent performance of DyTox and DyTox+ are clearly exposed.


\label{sec:ablations}
\noindent\textbf{Model ablations:} We report the step average accuracy (``\textit{Avg}'') and final step accuracy (``\textit{Last}'') over all seen classes in \autoref{tab:ablation} for the different ablations of our model DyTox on the challenging setting of CIFAR100 made of 50 steps. \alexd{We designed our transformer shallow (6 blocks) to have a comparable parameters count to other baselines, but also made it wider than usual "tiny" models \cite{dosovitskiy2020vit,touvron2021deit,touvron2021cait} (384d). This formulation proved to be already efficient to handle forgetting.}{cela doit être au moment où tu définis tes structures hyperparams, et certainement pas ici} We further add to this baseline transformer a naive knowledge distillation \cite{hinton2015knowledge_distillation} and a finetuning \cite{castro2018end_to_end_inc_learn,hou2019ucir,douillard2020podnet,yan2021der} applied after each task on a balanced set of new data and rehearsal data.
Finally, our DyTox strategy exploits directly the very nature of transformers (separated task information from the pixels information) to tackle catastrophic forgetting: it is made of three components: (1) a task token expansion, (2) a divergence classifier, and (3) independent classifiers \alex{trop descriptif, pas assez analytique, cette énumeration n'apporte pas d'infos en plus que la table}. All three greatly improve over the baseline transformer ($42.21\% \rightarrow 52.34\%$ in ``All'') while having almost no memory overhead. The independent classifiers with the sigmoid activations reduce the Chaudhry et al.'s \alex{bizarre cette citation, vraiment nécessarire le et al. ici ? }forgetting \cite{chaudhry2018riemannien_walk} by more than 8 percentage points (p.p.).


\input{tables/ablations}

\input{tables/plus}
\alex{bizarre maintenant, à introduire en même temps que le mixup je pense}
\noindent\textbf{Training procedure introspection:} We also compared the performances of the DyTox vs DyTox+ strategies in \autoref{tab:training_plus}: MixUp slightly improves by 1.39 p.p. the accuracy in joint learning (no continual, 1 step), but greatly improves in CIFAR100 50 steps by improving by 4.75 p.p. To further illustrate the fact, that DyTox+ doesn't simply improve raw performance, we also report the Chaudhry's forgetting \cite{chaudhry2018riemannien_walk} \alex{cette mesure est déjà défnie juste au dessus} which compares how performances dropped compared to previous steps. DyTox+ reduces this forgetting measure by 1.65 p.p.

\label{sec:memory_overhead}
\alex{t'en parles partout dans  les parties précedentes; faut regrouper ça. Là tu n'as aucune table, donc c'est plutôt dans implementation details ?}
\noindent\textbf{Memory Overhead:} Our DyTox strategy has for overhead, compared to a baseline transformer, a vector of size $+\mathbb{D}$ per task. In our case, $\mathbb{D}=384$ and the base model has $\sim11$M parameters, thus the overhead in memory is only of $+0.03\%$ per task. Given the challenging setting of CIFAR100 with 50 tasks, our memory overhead is still small ($+1.74\%$).

\label{sec:comp_over}
\alex{t'en parles partout dans  les pargrapgras précedents; faut regrouper ça}
\noindent\textbf{Computational Overhead:} The vast majority of the computation, done in the SABs, is shared among all tasks. The dynamical component of our model is located at the ultimate TAB. Moreover, the Task-Attention, contrary to the Self-Attention, has a time complexity linear in terms of tokens and not quadratic further reducing the time overhead to an acceptable amount. Overall, for each new task, one forward pass takes $2.24\%$ more time w.r.t the base transformer speed.

%\input{tables/sam}

%\input{tables/aug}
%\input{tables/ens_ablation}
%\input{tables/archi}
%\input{tables/old_sam}
%\input{tables/transf}

==> tables/archi.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}ll|cc|ccc|ccc|@{}}
\toprule
\textbf{Backbone} & \textbf{Methods} & \multicolumn{2}{c}{Joint (1 step)} & \multicolumn{2}{c}{0-10 (10 steps)} & \multicolumn{2}{c}{0-2 (50 steps)}\\
 & & \textbf{Final} & \textbf{Avg} & \textbf{Final} & \textbf{Avg} & \textbf{\%}  & \textbf{Final} & \textbf{Avg} & \textbf{\%}\\
\midrule
%\multirow{2}{*}{Thin ResNet34 (0.47m)} & AutoKD &  & -  &  &  &  & \\
%                          & \,+Mixup+Cutmix &  & -  &  &  &  & \\
%\midrule
\multirow{2}{*}{ResNet18 (11.2m)} & AutoKD & 71.50 & - & 45.51 & 65.95 & 63.36 & 38.31 & 62.82 & 53.54\\
                          & \,+Mixup+Cutmix & 73.88 & - & 50.34 & 69.44 & 68.13 & 48.23 & 68.74 & 65.28\\
\midrule
\multirow{2}{*}{Transf. (10.2m)} & AutoKD & 74.28 & -  & 48.56 & 66.92 & 65.37 & 39.47 & 61.40 & 53.13\\
                          & \,+Mixup+Cutmix & 78.23 & - & 51.27 & 70.48 & 65.51 & 47.88 & 68.51 & 61.21\\
\midrule
\multirow{2}{*}{Inception3 (22.3m)} & AutoKD & 80.84 & -  & 52.22 & 71.02 & 65.27 & & & \\
                          & \,+Mixup+Cutmix & 83.51 & - & 58.52 & 75.53 & 69.81 & & \\
\midrule
%\multirow{2}{*}{VGG16BN (134.6m)} & AutoKD &  & -  &  &  &  & \\
%                          & \,+Mixup+Cutmix &  & -  &  &  &  & \\
%\midrule
\multirow{2}{*}{ResNet50 (23.7m)} & AutoKD & 75.02 & -  & 46.71 & 65.85 & 62.28 & &  & \\
                          & \,+Mixup+Cutmix & 77.05 & -  & 51.89 & 68.45 & 66.23 & &  & \\
\midrule
\multirow{2}{*}{ResNext50 (23.2m)} & AutoKD & 76.27 & -  & 46.52 & 65.98 & 60.34 & &  & \\
                          & \,+Mixup+Cutmix & 76.54 & -  & 51.24 & 68.57 & 67.32 & & &\\
\midrule
\multirow{2}{*}{WideResNet50 (67.03m)} & AutoKD & 75.84 & -  & 48.99 & 68.33 & 64.47 &&  & \\
                          & \,+Mixup+Cutmix & 78.42 & -  & 54.26 & 71.06 & 69.10 & && \\
\midrule
\multirow{2}{*}{SEResNet18 (11.8m)} & AutoKD & 61.15 & -  & 33.4 & 53.63 & 54.61 & &  & \\
                          & \,+Mixup+Cutmix & 61.11 & -  & 35.44 & 54.91 & 57.99 & &  & \\
\midrule
\multirow{2}{*}{VGG16 (134.67m)} & AutoKD & 66.33 & - & 43.00 & 60.72 & 64.82 & & &\\
                                & \,+Mixup+Cutmix & 64.65 & - & 48.78 & 64.86 & 75.43 & & &\\
\midrule
\multirow{2}{*}{VGG16Bn (134.67m)} & AutoKD & 71.12 & - & 47.43 & 66.07 & 66.69 & & & \\
                                  & \,+Mixup+Cutmix & 67.85 & - & 53.21 & 68.72 & 78.42 & & &\\
\bottomrule
\end{tabular}
\caption{Effect of Mixup + Cutmix, resnet18 (11.2m), transf. (10.2m)}
\label{tab:cifar100-aug}
\end{table*}


==> tables/aug.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}ll|cc|cc|cc|@{}}
\toprule
\textbf{Backbone} & \textbf{Methods} & \multicolumn{2}{c}{Joint (1 step)} & \multicolumn{2}{c}{0-10 (10 steps)} & \multicolumn{2}{c}{0-2 (50 steps)}\\
 & & \textbf{Final} & \textbf{Avg} & \textbf{Final} & \textbf{Avg}  & \textbf{Final} & \textbf{Avg}\\
\midrule
\multirow{3}{*}{ResNet18} & AutoKD & - & 71.50 & 45.51 & 65.95 & 38.31 & 62.82\\
                          & \,+Mixup & - & 72.72  & 46.56 & 67.23 & 43.91 & 66.30\\
                          & \,+Mixup+Cutmix & - & 73.88 & 50.34 & 69.44 & 48.23 & 68.74\\
\midrule
\multirow{4}{*}{Transf.} & AutoKD & - & 74.28  & 48.56 & 66.92 & 39.47 & 61.40\\
                          & \,+Mixup & - & 76.50  & 50.02 & 68.33 & 47.73 & 68.33\\
                          & \,+Mixup+Cutmix & - & 78.23 & 51.27 & 70.48 & 47.88 & 68.51\\
\midrule
\multirow{2}{*}{Transf.} & Base & - & 74.28  & 43.41 & 63.87 & & \\
                          & \,+Mixup+Cutmix & - & 78.23 & 50.29 & 69.82 & &\\
\midrule
\multirow{2}{*}{Transf. w/ clf reset} & AutoKD & - &   & 8.93 & 33.76 & & \\
                          & \,+Mixup+Cutmix & - &  & 7.07 & 31.02 & &\\
\bottomrule
\end{tabular}
\caption{Effect of Mixup + Cutmix, resnet18 (11.2m), transf. (10.2m)}
\label{tab:cifar100-aug}
\end{table*}


==> tables/cifar100_b50.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}l|cc|cc|cc|@{}}
\toprule
\textbf{Methods} & \multicolumn{2}{c}{50-25 (3 steps)} & \multicolumn{2}{c}{50-10 (6 steps)} & \multicolumn{2}{c}{50-5 (11 steps)}\\
  & \textbf{\#P} & \textbf{Avg} &  \textbf{\#P} & \textbf{Avg} & \textbf{\#P} & \textbf{Avg} \\
\midrule
%ResNet18 Joint &  11.2 & - & 77.22 & 11.2 & - & 79.89 & 11.2 & - & 79.91\\
%Transf. Joint & 10.7 & - & 76.12 & 10.7 & - & 76.12 & 10.7 & - & 76.12\\
\midrule
iCaRL & 11.2 & 71.33\scriptsize{\mypm0.35} & 11.2 & 65.06\scriptsize{\mypm0.53} &  11.2 & 58.59\scriptsize{\mypm0.95}\\
UCIR  & 11.2 & 67.21\scriptsize{\mypm0.35} & 11.2 & 64.28\scriptsize{\mypm0.19} & 11.2 & 59.92\scriptsize{\mypm2.40}\\
BiC & 11.2 & 72.47\scriptsize{\mypm0.99} & 11.2 & 66.62\scriptsize{\mypm0.45} & 11.2 & 60.25\scriptsize{\mypm0.34}\\
WA  & 11.2 & 71.43\scriptsize{\mypm0.65} & 11.2 & 64.01\scriptsize{\mypm1.62} & 11.2 & 57.86\scriptsize{\mypm0.81} \\
PODNet  & 11.2 & 71.30\scriptsize{\mypm0.46} &  11.2 & 67.25\scriptsize{\mypm0.27}  & 11.2 & 64.04\scriptsize{\mypm0.43} \\
DER w/o Pruning  & 61.6 & 74.61\scriptsize{\mypm0.52} &  117.6 & 73.21\scriptsize{\mypm0.78} & 285.6 & 72.81\scriptsize{\mypm0.88}\\ % no pruning
%DER \cite{yan2021der}  & 4.96 & 74.57\scriptsize{\mypm0.42} & & 7.21 & 72.60\scriptsize{\mypm0.78} & 66 & 10.15 & 72.45\scriptsize{\mypm0.76} & 65\\
\midrule
%\multirow{1}{*}{Transf.} & AutoKD & - & - & 10.7 & 66.92 & - & - & 10.7 & 61.40\\
%\multirow{2}{*}{Transf. v2} & AutoKD & - & - & 10.7 & 68.69 & - & - & 10.7 & \tbd\\
%                            & \,+EnsCls & - & - & 10.7 & 69.88 & - & - & 10.7 & \tbd\\
DyTox & 10.684 & 72.11\mysmpm{0.31} &  10.685 & 70.01\mysmpm{0.10} &  10.687 & 66.82\mysmpm{0.17}\\
%DyTox+ & 10.684 & 71.81\mysmpm{0.27} & 64.22\mysmpm{0.30} & 10.685 & 69.40\mysmpm{0.32} & 61.78\mysmpm{0.45} & 10.687 & 67.11\mysmpm{0.36} & 59.40\mysmpm{0.33}\\
%DyTox++ & 10.684 & 71.82\mysmpm{0.21} & 65.01\mysmpm{0.09} & 10.685 & 69.23\mysmpm{0.23} & 62.74\mysmpm{0.46} & 10.687 & 67.36\mysmpm{0.21} & 60.64\mysmpm{0.02}\\
\bottomrule
\end{tabular}
\caption{Results on CIFAR100 with a large initial step of 50 classes. We report the results averaged over three different class orders.}
\label{tab:cifar100-b50}
\end{table*}

==> tables/ens_ablation.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}ll|ccc|ccc|@{}}
\toprule
\textbf{Backbone} & \textbf{Methods} & \multicolumn{2}{c}{0-10 (10 steps)} & \multicolumn{2}{c}{0-2 (50 steps)}\\
 & & \textbf{\#Params} & \textbf{Avg} & \textbf{Final}  & \textbf{\#Params} & \textbf{Avg} & \textbf{Final}\\
\midrule
ResNet18 & Joint & 11.2 & - & 80.41 & 11.2 & - 81.74\\
Transf. & Joint & 10.7 & - & 74.28 & 10.2 & - & 74.28\\
\midrule
\multirow{2}{*}{ResNet18} & WA \cite{zhao2020weightalignement} & 11.2 & 69.46 &  - & 11.2 & 64.32 & - \\
                          & DER \cite{yan2021der} & 4.96 & 74.64 & - & 10.15 & 72.05 & -\\
\midrule
\multirow{2}{*}{Transf.} & AutoKD & 10.7 & 66.92 & 48.56 & 10.2 & 61.40 & 39.47\\
                         & \,+Ens Cls & 10.7 & 65.23 & 47.13 &  & & \\
                         & \,+Freeze old tokens & & 65.14 & 46.61 & & &\\
                         & \,+Ft Freeze Sa CA & & 65.86 & 47.05 & & &\\
                         & \,+Ft Freeze Tokens & & 65.90 & 47.42 & & &\\
                         & \,+Head div1 & & 67.67 & 51.30 & & & \\
\bottomrule
\end{tabular}
\caption{CIFAR100-B0 benchmark}
\label{tab:cifar100-b0}
\end{table*}


==> tables/imagenet100_b50.tex <==
\begin{table*}[t]
	\begin{tabular}{l|ccccc}
	\toprule[0.3mm]
	\multirow{3}{*}{\textbf{Methods}} & \multicolumn{5}{c}{\textbf{ImageNet100 50-10 (6 steps)}}  \\ \\
			\cmidrule{2-6}
			 & \multirow{2}{*}{\textbf{$\#$P}} & \multicolumn{2}{c}{\textbf{top-1}}  & \multicolumn{2}{c}{\textbf{top-5}}  \\
			 \cmidrule{3-6}
			 &        & \textbf{Avg}          & \textbf{Last}    & \textbf{Avg} & \textbf{Last}   \\
			 \midrule
			ResNet18 Joint & $11.2$ & $81.20$ & $81.5$ & - & - \\
			Transf. Joint & 11.011 & - & 79.12 & - & 93.48\\
			%\,+ mixup & 11.011 & - & 81.82 & - & 94.72\\
			%\,+ sam & 11.011 & - & 82.62 & - & 95.94\\
			\midrule
			UCIR \cite{hou2019ucir} & $11.2$ & $68.09$ & $57.3$ & -& - \\
			PODNet \cite{douillard2020podnet} & $11.2$ & $74.33$ & - & -& -\\
			TPCIL\cite{tao2020tpcil} & $11.2$ & $74.81$ & $66.91$ & - & - \\ 
			DER \cite{yan2021der} & 67.20 & 78.20 & 74.92   & 94.20    & 91.30 \\ % no pruning
			%DER \cite{yan2021der} & 8.87  & 77.73 & 72.06 & 94.01    & 91.64 \\
			\midrule
			DyTox & 11.01 & 75.52 & 68.42 & 92.18 & 89.04\\ 
			%DyTox+ & 11.014 & 75.58 & 69.95 & 91.36 & 88.18\\
			%DyTox++ & 11.014 & 76.52 & 71.48 & 92.33 & 89.96\\
	\bottomrule[0.3mm]
	\end{tabular}
\caption{\fontsize{10}{12}\selectfont{Results on ImageNet-100  and ImageNet-1000 datasets.\textbf{Left}: The results on ImageNet100-B0 and ImageNet1000-B0 benchmark. \textbf{Right}: The results on ImageNet100-B50 benchmark. \emph{$\#$Paras} means the average number of parameters during inference over steps, which is counted by million. \emph{Avg} means the average accuracy ($\%$) over steps. \emph{Last} is the accuracy ($\%$) of the last step. \emph{Ours(w/o P)} means our method without pruning.}}
	\label{tab:imagenet}
\end{table*}




==> tables/nb_dim.tex <==
\begin{table}[t]
\centering
%\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}c|c|ccc@{}}
\hline
& Joint (1 steps) & \multicolumn{3}{c}{50 steps}  \\
\textbf{Embed dim} & \textbf{Last} ($\uparrow$) & \textbf{\#P} & \textbf{Last} ($\uparrow$) & \textbf{Forg.} ($\downarrow$)\Bstrut\\
\hline
192 & 73.63 & 2.68 & 52.92 & 28.00 \\
384 & 76.12 & 10.77 & 52.34 & 33.15 \\
444 &  73.47 & 14.27 & 52.15 & 32.84 \\
504 &  74.13 & 18.38 & 51.42 & 34.64 \\
768 & 75.30 & 42.60 & 51.13 & 35.78 \\
%960 & 74.80 & \\
\hline
\end{tabular}
%}
\caption{\textbf{Number of heads influence on continual} for the joint (1 step, no continual) and 50 steps settings on CIFAR100.
%We report the ``Last'' accuracy and forgetting \cite{chaudhry2018riemannien_walk}.
We choose a 5 blocks of SAB for our main experiments.}
\label{tab:nb_sab}
\end{table}

==> tables/nb_heads.tex <==
\begin{table}[t]
\centering
%\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}c|c|cc@{}}
\hline
& Joint (1 steps) & \multicolumn{2}{c}{50 steps}  \\
\textbf{\# Heads} & \textbf{Last} ($\uparrow$) & \textbf{Last} ($\uparrow$) & \textbf{Forg.} ($\downarrow$)\Bstrut\\
\hline
6 & 73.95 & 51.36 & 33.44 \\
12 & 76.12 & 52.34 & 33.15 \\
24 & 75.05 & 53.03 & 32.05 \\
\hline
\end{tabular}
%}
\caption{\textbf{Number of heads influence on continual} for the joint (1 step, no continual) and 50 steps settings on CIFAR100.
%We report the ``Last'' accuracy and forgetting \cite{chaudhry2018riemannien_walk}.
We choose a 5 blocks of SAB for our main experiments.}
\label{tab:nb_sab}
\end{table}

==> tables/nb_sab.tex <==
\begin{table}[t]
\centering
%\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}c|c|ccc@{}}
\hline
& Joint (1 steps) & \multicolumn{3}{c}{50 steps}  \\
\textbf{\# SAB} & \textbf{Last} ($\uparrow$) & \textbf{\#P} & \textbf{Last} ($\uparrow$) & \textbf{Forg.} ($\downarrow$)\Bstrut\\
\hline
4 & 74.71 & 8.91 & 51.76 & 32.60 \\
5 & 76.12 & 10.77 & 52.34 & 33.15 \\
6 & 76.06 & 12.45 & 51.28 & 35.12 \\
7 & 76.05 & 14.23 & 50.82 & 35.91 \\
\hline
\end{tabular}
%}
\caption{\textbf{Encoder depth influence on continual} for the joint (1 step, no continual) and 50 steps settings on CIFAR100.
%We report the ``Last'' accuracy and forgetting \cite{chaudhry2018riemannien_walk}.
We choose a 5 blocks of SAB for our main experiments.}
\label{tab:nb_sab}
\end{table}

==> tables/nb_tab.tex <==
\begin{table}[t]
\centering
%\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}c|c|ccc@{}}
\hline
& Joint (1 steps) & \multicolumn{3}{c}{50 steps}  \\
\textbf{\# TAB} & \textbf{Last} ($\uparrow$) & \textbf{\#P} & \textbf{Last} ($\uparrow$) & \textbf{Forg.} ($\downarrow$)\Bstrut\\
\hline
1 & 76.12 & 10.77 & 52.34 & 33.15 \\
2 & 75.04 & 12.45 & 52.69 & 34.11 \\
3 & 74.62 & 14.23 & 52.26 & 35.69 \\
\hline
\end{tabular}
%}
\caption{\textbf{Decoder depth influence on continual} for the joint (1 step, no continual) and 50 steps settings on CIFAR100.
%We report the ``Last'' accuracy and forgetting \cite{chaudhry2018riemannien_walk}.
We choose a 5 blocks of SAB for our main experiments.}
\label{tab:nb_sab}
\end{table}

==> tables/old_sam.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}ll|ccc|ccc|@{}}
\toprule
\textbf{Backbone} & \textbf{Methods} & \multicolumn{2}{c}{0-10 (10 steps)} & \multicolumn{2}{c}{0-2 (50 steps)}\\
 & & \textbf{\#Params} & \textbf{Avg} & \textbf{Final}  & \textbf{\#Params} & \textbf{Avg} & \textbf{Final}\\
\midrule
ResNet18 & Joint & 11.2 & - & 80.41 & 11.2 & - 81.74\\
Transf. & Joint & 10.2 & - & 74.28 & 10.2 & - & 74.28\\
\midrule
\multirow{2}{*}{ResNet18} & WA \cite{zhao2020weightalignement} & 11.2 & 69.46 &  - & 11.2 & 64.32 & - \\
                          & DER \cite{yan2021der} & 4.96 & 74.64 & - & 10.15 & 72.05 & -\\
\midrule
\multirow{2}{*}{Transf.} & AutoKD & 10.2 & 66.92 & 48.56 & 10.2 & 61.40 & 39.47\\
                         & \,Sam 0.2adapt inclr5e-5 & & 65.30 & 48.07 &  & & &\\
                         & \,Sam 0.05 inclr5e-5 & &  &  &  &  &62.61 & 44.82\\
\bottomrule
\end{tabular}
\caption{CIFAR100-B0 benchmark}
\label{tab:cifar100-b0}
\end{table*}


==> tables/pod.tex <==
\begin{table*}[t]
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{}l|cc}
\hline
 & \multicolumn{2}{c}{50 classes + 25 $\times$ 2 classes} \\
\textbf{Model}   & \textbf{Avg} & \textbf{Last}\\
\hline
DyTox-resnet & 54.24 & 42.66\\
DyTox-resnet + POD & 54.66 & \textbf{44.38}\\
DyTox-resnet + Local POD & \textbf{54.74} & 43.25\\
\hline
\end{tabular}
}
\caption{FOO}
\label{tab:cifar100-b0}
\end{table*}

==> tables/sam.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}ll|cc|cc|cc@{}}
\toprule
\textbf{Backbone} & \textbf{Sam?} & \multicolumn{2}{c}{Joint} & \multicolumn{2}{c}{0-10 (10 steps)} & \multicolumn{2}{c}{0-2 (50 steps)}\\
 & & \textbf{Avg} & \textbf{Final}  & \textbf{Avg} & \textbf{Final} &  \textbf{Avg} & \textbf{Final}\\
\midrule
Transf. & \xmark & --- & 76.48 & 72.30 & 57.70 & 65.95 & 47.21 \\
Transf. & \cmark & --- & 76.12 & 74.00 & 60.26 & 69.96 & 52.86 \\
\bottomrule
\end{tabular}
\caption{CIFAR100-B0 benchmark}
\label{tab:cifar100-b0}
\end{table*}


==> tables/transf.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}cccccc|c|ccc|ccc|@{}}
\toprule
\textbf{Embed} & \textbf{Depth} &  \textbf{Local} & \textbf{\# Heads} & \textbf{Patch} & \textbf{\#Params} & Joint & \multicolumn{3}{c}{Base} & \multicolumn{3}{c}{EnsCls}\\
 &&&&&& \textbf{Final} & \textbf{Avg} & \textbf{Final} & \textbf{\% of Joint}  & \textbf{Avg} & \textbf{Final} & \textbf{\% of Joint}\\
\midrule
192 & 6 & 4 & 12 & 4 & 2.7 & 72.98 & 66.82 & 49.21 & \green{67.43} & 64.89 & 47.33 & 64.85\\
336 & 8 & 4 & 12 & 4 & 10.9 & 71.56 & 64.73 & 45.11 & 63.04 & 63.54 & 44.03 & 61.53\\
336 & 8 & 6 & 12 & 4 & 10.9 & \green{75.39} & 67.61 & \green{50.17} & 66.55 & 65.95 & 47.34 & 62.79\\
384 & 6 & 3 & 12 & 4 & 10.7 & 72.17 & 64.79 & 45.39 & 62.89 & 62.72 & 43.72 & 60.58\\
384 & 6 & 4 & 3 & 4 & 10.7 & 70.62 & 62.57 & 44.03 & 62.35 & 61.70 & 42.84 & 60.66\\
384 & 6 & 4 & 6 & 4 & 10.7 & 73.78 & 66.13 & 47.43 & 64.29 & 64.79 & 45.51 & 61.68\\
384 & 6 & 4 & 12 & 4 & 10.7 & 74.28 & 66.96 & 48.20 & 64.89 & 65.26 & 46.61 & 62.75\\
384 & 6 & 4 & 12 & 6 & 10.7 & 69.98 & 62.81 & 44.64 & 63.79 & 61.00 & 42.19 & 60.29\\
384 & 6 & 4 & 24 & 4 & 10.7 & 74.29 & 66.95 & 48.24 & 64.93 & 65.09 & 46.07 & 62.01\\
384 & 6 & 5 & 12 & 4 & 10.7 & \red{76.33} & \red{68.69} & \red{50.70} & 66.42 & \red{69.88} & \red{52.74} & \red{69.09}\\
420 & 6 & 4 & 12 & 4 & 12.8 & 74.22 & 66.94 & 48.43 & 65.25 & 65.32 & 46.54 & 62.71\\
420 & 5 & 4 & 12 & 4 & 10.6 & \green{75.52} & \red{68.90} & \red{50.86} & \green{67.34} & 69.04 & 51.31 & 67.94\\
420 & 6 & 5 & 12 & 4 & 12.8 & 76.21 & 68.52 & 50.00 & 65.60 & \red{69.77} & \red{52.18} & \green{68.46}\\
480 & 4 & 2 & 6 & 4 & 11.2 & 69.97 & 62.15 & 42.68 & 61.0 & 61.32 & 42.08 & 60.14\\
480 & 4 & 2 & 12 & 4 & 11.2 & 71.74 & 63.09 & 44.88 & 62.56 & 62.85 & 43.71 & 60.93\\
480 & 4 & 2 & 24 & 4 & 11.2 & 71.27 & 63.93 & 44.78 & 62.83 & 62.76 & 43.61 & 61.19\\
480 & 4 & 3 & 6 & 4 & 11.2 & 73.68 & 66.76 & 48.53 & 65.87 & 67.35 & 48.57 & 65.92\\
480 & 4 & 3 & 12 & 4 & 11.2 & 74.43 & \green{68.43} & \green{50.47} & \red{67.81} & \green{68.13} & \green{49.91} & \green{67.06}\\
480 & 4 & 3 & 24 & 4 & 11.2 & \green{75.12} & \green{68.40} & \green{50.31} & 66.97 & \green{68.09} & \green{49.91} & 66.44\\


\bottomrule
\end{tabular}
\caption{CIFAR100-B0 benchmark 10 steps (10 inc), \red{best}, \green{second best}. base transformer vs Ensembling with class token (EnsCLs)}
\label{tab:cifar100-b0}
\end{table*}

